Generalized Max Pooling

State-of-the-art patch-based image representations involve a pooling operation that aggregates statistics computed from local descriptors. Standard pooling operations include sum- and max-pooling. Sum-pooling lacks discriminability because the resulting representation is strongly influenced by frequent yet often uninformative descriptors, but only weakly influenced by rare yet potentially highly-informative ones. Max-pooling equalizes the influence of frequent and rare descriptors but is only applicable to representations that rely on count statistics, such as the bag-of-visual-words (BOV) and its soft- and sparse-coding extensions. We propose a novel pooling mechanism that achieves the same effect as max-pooling but is applicable beyond the BOV and especially to the state-of-the-art Fisher Vector -- hence the name Generalized Max Pooling (GMP). It involves equalizing the similarity between each patch and the pooled representation, which is shown to be equivalent to re-weighting the per-patch statistics. We show on five public image classification benchmarks that the proposed GMP can lead to significant performance gains with respect to heuristic alternatives.

==> general.tex <==
\section{A Direct Solution}
\label{sec:general}

We now provide a new formulation of equation (\ref{eqn:dual})
which we refer to as the primal formulation because it only depends on $\p$.
%\ie we now assume that we have access to $\p$.
%We offer its matching interpretation and exibit a closed form solution to the problem.
%%We then show that, in the case of the BOV, the proposed framework leads to the popular max-pooling.
%We subsequently discuss the practical problem of computing the solution to the primal problem.
%%We finally discuss the case $\rho \neq 0$.
%
%\subsection{A direct solution}
Since $K$ is a PSD matrix, it rewrites as
%
\begin{equation} \label{eqn:psd}
K = \Phi^T \Phi,
\end{equation}
%
with $\Phi$ the $D \times M$ matrix
that contains the $D$-dimensional patch embeddings: $\Phi = [\p(x_1), ..., \p(x_M)]$.
%Note that, since in practice we have to rely on finite-dimensional embeddings,
%equation (\ref{eqn:psd}) may only be approximate.
Hence we can rewrite equation (\ref{eqn:dual}) as
%
\begin{equation}
\Phi^T \Phi w = \1_M.
\end{equation}
%
We introduce the notation $\p = \Phi w$.
We have $\p = \sum_{i=1}^M w_i \p(x_i)$,
\ie $\p$ is the weighted-pooled representation we are trying to compute.
Therefore, we seek $\p$ that optimizes
%
\begin{equation} \label{eqn:primal}
\Phi^T \p = \1_M.
\end{equation}
%
An advantage of the primal formulation is that it offers a {\em matching interpretation}:
matching a single patch embedding $\p(x_i)$ with the weighted representation
should result in a similarity equal to 1, for all descriptors $x_i$.
%Hence, all patches ...
Another advantage is that, 
instead of first computing a set of weights and then combining the per-patch embeddings, 
we can {\em compute directly the weighted image representation}.
In general, equation (\ref{eqn:primal}) might not have a solution or it might have multiple solutions.
Therefore, we turn (\ref{eqn:primal}) into a least-squares regression problem and seek
%
\begin{equation} \label{eqn:primal_ls}
\p^* = \arg \min_\p ||\Phi^T \p - \1_M||^2,
\end{equation}
%
with the additional constraint that $\p^*$ has minimal norm in the case of an infinite number of solutions.
%We formulate problem (\ref{eqn:lineareq}) as a least-squares regression problem.
%and introduce a regularization term to avoid the problematic cases where the system of equations either does not
%admit any exact solution or admits multiple solutions. 
%We therefore solve:
%%
%\begin{equation} \label{eqn:primal}
%\p^* = \arg \min_\p \frac{1}{2M} \sum_{i=1}^M (\p_i^T \p - 1)^2 % + \frac{\lbd}{2} ||\p||^2
%\end{equation}
%%
The previous problem admits a simple closed-form solution:
%Then the minimum-norm solution to (\ref{eqn:primal}) has a simple closed form formula:
%
\begin{equation} \label{eqn:primalsol}
\p^* = (\Phi^T)^+ \1_M =  (\Phi \Phi^T)^+ \Phi \1_M,
\end{equation}
%
where $^+$ denotes the pseudo-inverse
and the second equality stems from the property $A^+=(A^TA)^+A^T$.
%by setting $A=\Phi^T$, we can rewrite equation (\ref{eqn:primalsol1}) as:
%%
%\begin{equation} \label{eqn:primalsol}
%\p^* = (\Phi \Phi^T)^+ \Phi \1_M
%\end{equation}
%%
We note that $\Phi \1_M = \sum_{i=1}^M \p(x_i)$ is the sum-pooled vector 
of embeddings which is equivalent to the average-pooled vectors since
we $\ell_2$-normalize our final image descriptors. 
Hence, the proposed weighted-pooling mechanism involves projecting 
the average-pooled vector $\Phi \1_M$ on $(\Phi \Phi^T)^+$.
%Note that this is different from recent works in computer vision advocating for
%the decorrelation of the data \cite{jegou12pca,hariharan12lda}
%since in our case $C$ is computed {\em from patches of the same image}.

Since the pseudo-inverse is not a continuous operation 
%(in the sense that if the sequence of matrices $A_n$ converges
%to $A$, then the sequence $A_n^+$ does not necessarily converge to $A^+$),
it is generally beneficial to add a regularization term to obtain
a stable solution. We introduce $\p^*_\lbd$:
%
\begin{equation} \label{eqn:primalreg}
\p^*_\lbd = \arg \min_\p ||\Phi^T \p - \1_M||^2  + \lbd ||\p||^2.
\end{equation}
%
This is a ridge regression problem whose solution is
%
\begin{equation} \label{eqn:primalsolreg}
\p^*_\lbd = (\Phi \Phi^T + \lbd I)^{-1} \Phi \1_M.
\end{equation}
%
The regularization parameter $\lbd$ should be cross-validated.
For $\lbd$ very large, we have $\p^*_\lbd \approx  \Phi \1_M / \lbd$
and we are back to average pooling.
Therefore, $\lbd$ does not only play a regularization role.
It also enables to smoothly transition between the solution (\ref{eqn:primalsol}) ($\lbd=0$)
and average pooling ($\lbd \rightarrow \infty$).

%\subsection{Computing $\p^*$}
We now turn to the problem of computing $\p^*_\lbd$ in practice.
We can compute (\ref{eqn:primalsolreg}) 
using Conjugate Gradient Descent (CGD)
which is designed for PSD matrices. % which may be sparse.
This might be computationally intensive if the embedding dimensionality $D$ 
is large and the matrix $\Phi$ is full.
However, the computation can be sped-up if the individual patch embeddings $\p(x_i)$ are block sparse. 
By block sparse we mean that 
the indices of the embedding can be partitioned into a set of groups where the activation
of one entry in a group means the activation of all entries in the group.
This is the case for instance of the VLAD and the SV where
each group of indices corresponds to a given cluster centroid.
This is also the case of the FV if we assume a hard assignment model
where each group corresponds to the gradients with respect to the parameters of a given Gaussian.
In such a case, the matrix $\Phi \Phi^T$ is block-diagonal. 
Consequently $\Phi \Phi^T + \lbd I$ is block diagonal
and (\ref{eqn:primalsolreg}) can be solved block-by-block,
which is significantly less demanding than solving the full problem directly.


==> probabilistic.tex <==
\section{Proposed Re-weighting Framework}\label{sec:prob}

Let $X = \{x_1, \ldots, x_M\}$ and 
$Y = \{y_1, \ldots, x_N\}$ denote two sets of local descriptors
extracted from two images.
%Let  $\p$ denote the coding function. % that embeds the descriptors into a typically higher-dimensional space.
Let $\p_X = \frac{1}{M} \sum_{i=1}^M \p(x_i)$ and $\p_Y = \frac{1}{N} \sum_{j=1}^N \p(y_j)$
denote the average-pooled representations.
The dot-product $K(X,Y) = \p_X^T \p_Y$ can be rewritten as a Sum Match Kernel (SMK): % \cite{}:
%
\begin{equation}
K(X,Y) = \frac{1}{MN}\sum^M_{i=1} \sum^N_{j=1} k(x_i,y_j),
\end{equation}
%
where $k(x_i,y_j) = \p(x_i)^T \p(y_j)$ is by definition a Positive Semi Definite (PSD) kernel.

For instance, in the BOV case, 
$\p(x)$ is a binary vector whose dimension is equal to the codebook size 
and with a single non-zero entry at the index of the closest centroid to descriptor $x$.
In this case, $k(x,y)=1$ if $x$ and $y$ fall in the same Voronoi region and 0 otherwise.

As another example, if $k$ is the Gaussian kernel 
$k_{\s}(x,y) \propto \exp(-\frac{||x-y||^2}{2\s^2})$,
the SMK is referred to as the Gaussian Match Kernel (GMK).
In such a case, the embedding $\p$ is obtained by combining random projections 
with cosine non-linearities thus leading to the EMK \cite{bo2009efficient}.

In what follows, we first focus on the GMK.
This is because the GMK has a probabilistic interpretation 
that we leverage to motivate our re-weighting scheme (section \ref{sec:gmk}).
%which we leverage to 
%We relate the GMK to probability product kernels between kernel density estimators.
%We subsequently propose a re-weighting scheme to treat burstiness for the GMK
We then propose a criterion to compute the weights
% is actually generic we focus on the dual formulation, 
that depends only on the kernel $k$ between individual descriptors and not on the embedding $\p$
(section \ref{sec:wgh}).
Therefore, the proposed weight computation algorithm can be extrapolated 
to any PSD kernel $k$ %and consequently to any embedding function $\p$,
even if it does not have a probabilistic interpretation.

\subsection{Probability product kernels} \label{sec:gmk}
We can derive from the two sets $X$ and $Y$ two Kernel Density Estimators (KDEs):
$p(x) = \frac{1}{M} \sum_{i=1}^M k_{\frac{\s}{\sqrt{2}}}(x,x_i)$ and 
$q(x) = \frac{1}{N} \sum_{j=1}^N k_{\frac{\s}{\sqrt{2}}}(x,y_j)$.
Given two probability distributions $p$ and $q$, 
the Probability Product Kernel (PPK) \cite{jebara2004probability} measures their similarity:
%
\begin{equation}
K^\rho_{ppk}(p,q)= \int p(x)^{\rho} q(x)^{\rho} dx,
\end{equation}
%
where $\rho$ is a parameter of the kernel.
When $\rho=1$, the PPK is known as the expected likelihood kernel 
%(because the kernel takes the form of the expectation of one distribution under the other)
and $\rho=1/2$ leads to the Bhattacharyya kernel.
The GMK between $X$ and $Y$ can be written as a PPK between $p$ and $q$:
%
\begin{eqnarray}
        K_{ppk}^1(p,q) = \frac{1}{MN}\sum^M_{i=1} \sum^N_{j=1} \int k_{\frac{\sigma}{\sqrt{2}}}(x,x_i) k_{\frac{\sigma}{\sqrt{2}}}(x,y_j) dx \nonumber \\
        \varpropto \frac{1}{MN}\sum^M_{i=1} \sum^N_{j=1} k_{\s}(x_i,y_j) = K_{gmk}(X,Y).
\label{eqn:patch_match}
\end{eqnarray}
%
This probabilistic view of the GMK provides a way to visualize the impact of similar descriptors.
Indeed, a group of similar descriptors in $X$,
will lead to a mode in the distribution $p$.
Figure~\ref{fig:gpr_eg} illustrates this effect, showing two groups of descriptors 
leading to a bi-modal probability distribution.
One solution to lessen the effect of frequent descriptors 
is to choose values $\rho < 1$ in the PPK as depicted in Figure~\ref{fig:gpr_eg}.
However, this solution faces two major problems.
First, for $\rho < 1$, the PPK between two KDEs can no longer be reduced to a SMK.
In such a case we cannot rewrite the costly kernel $K(X,Y)$ 
as an efficient dot-product.
Note that being able to write $K$ as a dot-product between pooled representations
enables us to learn efficient linear classifiers on these representations.
Second, if we want to perfectly equalize the modes, we need to set $\rho \rightarrow 0$.
In such a case, $p^\rho$ becomes flat and therefore uninformative.

%a principled solution to dealing with bursty elements.
%when measuring the similarity between two patches with a Gaussian kernel.
%Hence, a principled way to deal with frequent descriptors is to equalize such modes.

% which shows a bimodal 
%probability distribution raised to the power 0.5. 
%As $\rho \rightarrow 0$, the distributions flattens, 
%thus decreasing the relative importance of the modes.

%Moreover, evaluating the resultant integral is not straightforward. 
%Approximate techniques have been proposed to address the problem of computing the PPK between mixture models.
%The simplest one is to approximate the power of a sum as a sum of powers \cite{jebara2004probability}.
%However, this does not address the burstiness effect since each element of the sum is treated individually.
%%Note that the same effect can be obtained by cross-validating the value of $\s$ and that it does not address our burstiness problem.
%Another approach proposed for the Bhattacharyya kernel is to use a variational approximation \cite{hershey2008variational}.
%However, the reduction to a SMK is unfeasible for this method.


\subsection{Weighted pooling} \label{sec:wgh}
\begin{figure}[!t]
\centering
    \includegraphics[width=0.8\linewidth]{gpr_sigma3.00_lambda0.00_alpha0.00_pr0.pdf}
    \label{fig:gpr_gamma2pt00_sigma0pt00}
\caption{Probability distributions formed by KDE with no weights (KDE), 
after exponentiation to the power $\rho=0.5$ and renormalization ($\textrm{KDE}^{0.5}$), 
and with weights computed with the proposed approach (weighted KDE). 
The KDEs were generated using 5 1-dimensional observations (marked as black dots in the plot) 
with values $[-11, -10, 7, 8, 9]$.}
\label{fig:gpr_eg}
\end{figure}

To treat the issue of frequently-occurring descriptors, 
we propose to {\em re-weight their embeddings}.
For each descriptor $x_i$, we learn a weight $w_i$ and the weighted-pooled representation is $\sum_{i=1}^M w_i \p(x_i)$.
This has two major advantages with respect to the power alternative discussed in the previous paragraph. 
First, we can still express the kernel $K(X,Y)$ as a dot-product between (weighted-)pooled representations.
Second, we can equalize the modes without flattening the whole distribution.

%Once weights have been learned, 
%the pooled representation of $X$ can be rewritten as $\sum_{i=1}^M w_i \p(x_i)$.

%We now propose an alternative which mimicks the effect of the power transform but which still enables writing
%the embedding of a set as a linear combination of the individual elements.
%The proposed solution is based on the following simple observation:
%{\em while the power parameter $\rho$ impacts the relative weights of the modes, 
%it does not affect their locations in the descriptor space}.
%To achieve a similar effect to setting $\rho < 1$, 
%we propose to {\em linearly re-weight the descriptors}.
%Indeed linear re-weighting does not change the mode locations 
%but acts on their relative weights. 
%Once weights have been learned, 
%the pooled representation of $X$ can be rewritten as $\sum_{i=1}^M w_i \p(x_i)$.

Instead of exactly equalizing the modes -- which would require first detecting the modes,
a costly process -- we propose to {\em equalize the distribution at the position of each sample $x_i$}.
As shown on Figure \ref{fig:gpr_eg}, this has a similar effect.
That is, given a set of samples $X = \{x_1, \ldots, x_M\}$, 
we learn the vector of weights $w=[w_1, \ldots w_M]$ such that
%
\begin{equation} \label{eqn:flat}
\sum^M_{j=1} w_j k_{\s}(x_i,x_j) = c \text{ for } i=1 \ldots M,
\end{equation}
%
where $c$ is a constant value.
Note that the resulting weighted function is not necessarily a distribution 
in the sense that $\sum_{i=1}^M w_i$ might not sum to one.
However, we always assume that the final image representation is $\ell_2$-normalized.
This is consistent with the dot-product similarity (and therefore with the fact that we use linear kernel
machines for classification) as this enforces an image to be closest to itself.
This has also been shown to improve results \cite{perronnin2010improving}.
Therefore, we are only interested in computing $w$ up to a multiplicative factor
and we arbitrarily set the value $c=1$.

%In what follows, we focus on the case $\rho=0$.
%We underline that setting $\rho=0$ in (\ref{eqn:flat}) is different from raising the original unweighted
%distribution to the power 0 as the latter would lead to a flat unininformative distribution.
%As shown in Figure \ref{fig:gpr_eg}, even in the limit case $\rho =0$ the proposed criterion (\ref{eqn:flat}) 
%equalizes the likelihood of the samples but does not flatten the overall distribution,
%The general case $0 < \rho<1$ will be discussed later.
%this has the effect of equalizing  on the KDE.
Introducing $K$ the $M \times M$ kernel matrix between individual elements $x_i$, 
$w$ the $M \times 1$ vector of weights and $\1_M$ the $M \times 1$ vector of all ones, 
we rewrite equation (\ref{eqn:flat}) as
%
\begin{equation} \label{eqn:dual}
K w = \1_M.
\end{equation}
%
We note that equation (\ref{eqn:dual}) -- which we refer to as the dual formulation 
because it only depends on $k$ -- 
is generic and can be applied to any PSD kernel $k$.
However, there are two major limitations of this dual formulation.
First, its interpretability is unclear when it is applied beyond the GMK
since we generally do not have a probabilistic interpretation of SMKs.
Second, it requires computing the distance between all pairs of patch descriptors. % (cost in $O(M^2)$)
%and solving a system of $M$ equations with $M$ unknowns (cost in $O(M^2)$ too).
%While such a cost might be acceptable when the number of patch descriptors is not too large ({\em e.g.} on the order of 1K),
%obtaining state-of-the-art results in classification requires extracting tens-of-thousands of patches per image \cite{zhou10sv,chatfield11devil}.
%In such a case, the quadratic cost is not acceptable.
which is too costly when extracting tens of thousands of descriptors~\cite{zhou10sv,chatfield11devil}.
%We now provide a direct solution to problem~(\ref{eqn:dual}), 
%\ie instead of first computing the weights and then combining the embeddings in a weighted fashion,
%we compute directly the final representation.
%As explained in the next section, this primal formulation offers both a higher interpretability and, 
%for several encoding functions $\p$, a more efficient solution.

